Faster Algorithms for Optimal Ex-Ante Coordinated Collusive Strategies in Extensive-Form Zero-Sum Games

We focus on the problem of finding an optimal strategy for a team of two players that faces an opponent in an imperfect-information zero-sum extensive-form game. Team members are not allowed to communicate during play but can coordinate before the game. In that setting, it is known that the best the team can do is sample a profile of potentially randomized strategies (one per player) from a joint (a.k.a. correlated) probability distribution at the beginning of the game. In this paper, we first provide new modeling results about computing such an optimal distribution by drawing a connection to a different literature on extensive-form correlation. Second, we provide an algorithm that computes such an optimal distribution by only using profiles where only one of the team members gets to randomize in each profile. We can also cap the number of such profiles we allow in the solution. This begets an anytime algorithm by increasing the cap. We find that often a handful of well-chosen such profiles suffices to reach optimal utility for the team. This enables team members to reach coordination through a relatively simple and understandable plan. Finally, inspired by this observation and leveraging theoretical concepts that we introduce, we develop an efficient column-generation algorithm for finding an optimal distribution for the team. We evaluate it on a suite of common benchmark games. It is three orders of magnitude faster than the prior state of the art on games that the latter can solve and it can also solve several games that were previously unsolvable.

==> text/__latexindent_temp.tex <==
\section{A Formulation of TMECor Based on Extensive-Form Correlation Plans}

% Si dice che l'idea che introduciamo è di usare il politopo di correlazione invece della realization form.
%
% Svantaggi:
% - Più entries nel vettore
%
% Vantaggi:
% - oracolo di best response è molto più tight
% - vale una structural decomposition simile (vedi sotto)
%
% === Remark sul fatto che solo le relevant sequences appaiono, non tutte le coppie.
%
% Overall, i vantaggi superano decisamente gli svantaggi. Inoltre, nel resto del paper mostriamo come la nuova rappresentazione e l'oracolo possono essere usati in un algoritmo diverso da quello di NeurIPS 2019:
% - Small support
% - Column generation

%As discussed, the advantage of the {realization form} introduced by \citet{Farina18:Ex} resides in the fact that it compactly represents the correlated distribution of play $\mu\team$ of the team as a vector with as many components as leaves in the game. This is in stark contrast with the naive representation of $\mu\team$ as an vector in the probability simplex with support $\Pi\tone\times\Pi\ttwo$---a set with an exponential number of elements in general. However, despite that major benefit, it is not known how to effectively characterize the realization polytope. Hence, MIP oracles exploiting the realization form are of limited scalability (see~\cref{sec:exp}).

We propose using a different representation of the correlated distribution of play $\mu\team$, inspired by the growing body of literature on extensive-form correlated equilibria. Like the \textit{realization form} by \citet{Farina18:Ex}, in our approach we represent $\mu\team$ as a vector with only a polynomial number of components. However, unlike the realization form, the number of components scales  as the product of the number of sequences of the two players, which can be significantly larger than the number of leaves. This downside is amply outweighed by the following benefits.
%
First, we show that in practice our proposed representation of $\mu\team$ enables us to compute best responses for the team significantly faster than the prior representations.
%
Second, in certain classes of games, we even show that our proposed representation enables the computation of a TMECor in polynomial time. This is the case, for example, in Goofspiel, a popular benchmark game in computational game theory~\citep{Ross71:Goofspiel}.


\subsection{Extensive-Form Correlation Plans}

Our representation is based on the concept of \emph{extensive-form correlation plans}, introduced by \citet{Stengel08:Extensive} in their seminal paper on extensive-form correlation. In particular, we map the correlated distribution of play $\mu\team$ of the team to the vector $\vec{\xi}\team$ indexed over pairs of sequences $(\sigma\tone,\sigma\ttwo) \in \Sigma\tone\rele\Sigma\ttwo$, where each entry is defined as
\begin{equation}\label{eq:xi def}
	\xi\team[(\sigma\tone,\sigma\ttwo)]\defeq \sum_{\substack{\pi\tone\in\Pi\tone(\sigma\tone)\\\pi\ttwo\in\Pi\ttwo(\sigma\ttwo)}} \mu\team[(\pi\tone,\pi\ttwo)]. 
\end{equation}

Here $\vec{\xi}\team$ is not indexed over \emph{all} pairs  of sequences $(\sigma\tone,\sigma\ttwo)$---only \emph{relevant} sequence pairs. While there are games in which this distinction is meaningless (that is, games in which all sequences pairs for the team members are relevant), in practice the number of relevant sequence pairs is only a tiny fraction of the total number of sequence pairs, as shown in \cref{table:rele vs prod}(b).

\begin{table*}%[th]
    \centering
    \sisetup{scientific-notation=false,round-mode=places,
round-precision=2}
    \setlength{\tabcolsep}{4.0pt}\small\centering
    \begin{tikzpicture}
    \node[anchor=west] at (0,0) {
    \begin{tabular}{lrrrr|||rr|||ccc}
        \toprule
        \multirow{2}{*}{\makebox[.6cm]{~}\bf Game instance} & \multicolumn{3}{c}{\bf Num. sequences} & \bf Num. leaves & \multirow{2}{*}{\scriptsize{$\displaystyle\frac{|\Sigma\tone \rele \Sigma\ttwo|}{|Z|}$}} & \multirow{2}{*}{\scriptsize{$\displaystyle\frac{|\Sigma\tone \times \Sigma\ttwo|}{|\Sigma\tone \rele \Sigma\ttwo|}$}} & \multicolumn{3}{c}{\bf Triangle-free?} \\
        &$|\Sigma_1|$ & $|\Sigma_2|$ & $|\Sigma_3|$ & \multicolumn{1}{c}{$|Z|$}&&&\small$\opppl{}=1$&\small$\opppl{}=2$&\small$\opppl{}=3$\\
        \midrule
        \makebox[.6cm][l]{\textbf{[A]}}Kuhn poker (3 ranks) &\num{25}&\num{25}&\num{25} &  \num{78} & \num{3.3974} & \num{2.358} &\xmark&\xmark&\xmark\\
        \makebox[.6cm][l]{\textbf{[B]}}Kuhn poker (4 ranks) &\num{33}&\num{33}&\num{33} & \num{312} & \num{1.5929} & \num{2.1911} &\xmark&\xmark&\xmark \\
        \makebox[.6cm][l]{\textbf{[C]}}Kuhn poker (12 ranks) &\num{97}&\num{97}&\num{97} & \num{17160} & \num{0.288} & \num{1.9027} &\xmark&\xmark&\xmark\\
        \midrule
        \makebox[.6cm][l]{\textbf{[D]}}Goofspiel (3 ranks, limited info) & \num{934} & \num{934} & \num{934} & \num{1296} & \num{9.5355} & \num{70.588} &\cmark&\cmark&\cmark\\
        \makebox[.6cm][l]{\textbf{[E]}}Goofspiel (3 ranks) &\num{1630}&\num{1630}&\num{1630} & \num{1296} & \num{15.53} & \num{131.96} &\cmark&\cmark&\cmark \\
        \midrule
        \makebox[.6cm][l]{\textbf{[F]}}Liar's dice (3 faces) &\num{1021}&\num{1021}&\num{1021} & \num{13797} & \num{5.26} & \num{14.42} &\xmark&\xmark&\xmark \\
        \makebox[.6cm][l]{\textbf{[G]}}Liar's dice (4 faces) &\num{10921}&\num{10921}&\num{10921} & \num{262080} & \num{6.2518} & \num{72.79} &\xmark&\xmark&\xmark\\
        \midrule
        \makebox[.6cm][l]{\textbf{[H]}}Leduc poker (3 ranks, 1 raise) &\num{457}&\num{457}&\num{457} & \num{4500} & \num{2.6215} & \num{17.703568703907773} &\xmark&\xmark&\xmark\\
        \makebox[.6cm][l]{\textbf{[I]}}Leduc poker (4 ranks, 1 raise) & 801 &801&801 & 16908 & \num{1.338123964986988} & \num{28.358055248618785} &\xmark&\xmark&\xmark\\
        \makebox[.6cm][l]{\textbf{[J]}}Leduc poker (2 ranks, 2 raises) & 1443 & 1443 & 1443 & 3786 & \num{7.275488642366614} & \num{75.594445452895262} &\xmark&\xmark&\xmark\\
        %Leduc poker (3 raises) &\num{7687}&\num{7687}&\num{7687} & \num{81072} && \num{\xintfloateval{357802 / 81072}} & \num{\xintfloateval{59089969 / 357802}} &&\xmark&\xmark&\xmark \\
        \bottomrule
    \end{tabular}};
    \draw[line width=2.3mm,white] (10.54,-2.6) -- (10.54,2.6);
    \draw[line width=2.3mm,white] (14.28,-2.6) -- (14.28,2.6);
    \node[anchor=north] at (5.1,-2.55) {\textbf{(a)} --- Game instances and sizes};
    \node[anchor=north] at (12.5,-2.55) {\textbf{(b)}};
    \node[anchor=north] at (16.0,-2.55) {\textbf{(c)}};
    \end{tikzpicture}\vspace{-2mm}
    \caption{\textbf{(a)} Size of the game instances used in our experiments, in terms of number of sequences $|\Sigma_i|$ for each player $i$, and number of leaves $|Z|$.
    \textbf{(b)} Ratio between the number of leaves $|Z|$, number of sequence pairs for the team members $|\Sigma\tone \times \Sigma\ttwo|$, and number of \emph{relevant} sequence pairs for the team members $|\Sigma\tone \rele \Sigma\ttwo|$ in various benchmark games. For all games reported in the subtable, we chose the first two players to act as the team members. \textbf{(c)} The subtable reports whether the interaction of the team members is triangle-free \citep{Farina20:Polynomial}, given the opponent player \opppl{}.}
    \label{table:rele vs prod}\vspace{-3mm}
\end{table*}

The set of extensive-form correlation plans $\vec{\xi}\team$ that can be induced as $\mu\team$ varies over the set of all correlated distributions of play for the team members is a convex polytope. We denote it as $\Xi\team$ and call it the \emph{polytope of correlation plans}. We will recall existing results and provide new ones about the structure of $\Xi\team$ in \cref{sec:srcp}. 

\subsection{Computing a TMECor using Correlation Plans}

Extensive-form correlation plans encode a \emph{superset} of the information encoded by realization plans. Indeed,  for all $z$,
$\xi\team[\sigma\tone(z),\sigma\ttwo(z)] = \rho\team[z].$
Using the previous identity, we can rewrite the problem of computing a TMECor of a constant-sum game \eqref{eq:tmecor_basic} as
\[
    \argmax_{\vec{\xi}\team \in \Xi\team} \min_{\vec{y}\opp \in \Y\opp} \sum_{z\in Z} \hat{u}\team(z) \xi\team[\sigma\tone(z),\sigma\ttwo(z)] y[\sigma\opp(z)].
\]
By dualizing the inner linear minimization problem over $\vec{y}\opp$, we get the following proposition that shows that a TMECor can be found as the solution to a linear program (LP) with a polynomial number of variables. (All the proofs of this paper can be found in the appendix.)
\begin{restatable}{proposition}{proptmecorlp}\label{prop:tmecor as lp}
    An extensive-form correlation plan $\vec{\xi}\team$ is a TMECor if and only if it is a solution to the LP
    \begin{equation*}
        \mleft\{\hspace{-1.25mm}\begin{array}{l}
            \displaystyle
            %% OBJECTIVE
            \argmax_{\vec{\xi}\team}~~~ v_\emptyseq,\quad\text{\normalfont subject to:}\\
            %\text{\normalfont subject to:}\\
            %% CONSTRAINT 1
            ~\circled{\normalfont 1}~ \displaystyle v_I - ~\sum_{\mathclap{\substack{I' \in \mathcal{I}\opp\\\sigma\opp(I') = (I, a)}}}~ v_{I'} \le ~\sum_{\mathclap{\substack{z \in Z\\\sigma\opp(z) = (I,a)}}} \hat{u}\team(z)\xi\team[\sigma\tone(z),\sigma\ttwo(z)]\\[-4mm]
            \hspace{5cm}\forall\, (I,\!a) \!\in\! \Sigma\opp\!\!\setminus\! \{\emptyseq\}\\[2mm]
            %% CONSTRAINT 2
            ~\circled{\normalfont 2}~\displaystyle v_\emptyseq - ~\sum_{\mathclap{\substack{I' \in \mathcal{I}\opp\\\sigma\opp(I') = \emptyseq}}}~ v_{I'} \le ~\sum_{\mathclap{\substack{z \in Z\\\sigma\opp(z) = \emptyseq}}} \hat{u}\team(z)\xi\team[\sigma\tone(z),\sigma\ttwo(z)]\\[8mm]
            %% CONSTRAINT 3
            ~\circled{\normalfont 3}~v_\emptyseq\textnormal{ free}, v_{I} \textnormal{ free } \quad \forall\ I \in \mathcal{I}\opp\\[.5mm]
            %% CONSTRAINT 4
            ~\circled{\normalfont 4}~\vec{\xi}\team \in \Xi\team.
        \end{array}\mright.
    \end{equation*}
\end{restatable}

\noindent As a direct consequence of \cref{prop:tmecor as lp}, a TMECor can be found in polynomial time whenever $\Xi\team$ can be represented as the intersection of a set of polynomially many linear constraints. In \cref{sec:srcp}, we recall when that is the case.


